SILK: Smooth InterpoLation frameworK for motion in-betweening A Simplified Computational Approach

Motion in-betweening is a crucial tool for animators, enabling intricate control over pose-level details in each keyframe. Recent machine learning solutions for motion in-betweening rely on complex models, incorporating skeleton-aware architectures or requiring multiple modules and training steps. In this work, we introduce a simple yet effective Transformer-based framework, employing a single Transformer encoder to synthesize realistic motions for motion in-betweening tasks. We find that data modeling choices play a significant role in improving in-betweening performance. Among others, we show that increasing data volume can yield equivalent or improved motion transitions, that the choice of pose representation is vital for achieving high-quality results, and that incorporating velocity input features enhances animation performance. These findings challenge the assumption that model complexity is the primary determinant of animation quality and provide insights into a more data-centric approach to motion interpolation. Additional videos and supplementary material are available at https://silk-paper.github.io.

==> inputs/assets/figure_pca.tex <==

\begin{figure}[b]
  \centering
  \begin{subfigure}{0.23\textwidth}
    \centering
    \includegraphics[width=\textwidth, height=\textwidth, keepaspectratio]{figures/pca_root.png} % Specify width and maintain aspect ratio
    \caption{PCA -- Root Space}
    \label{fig:pca-root}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.23\textwidth}
    \centering
    \includegraphics[width=\textwidth, height=\textwidth, keepaspectratio]{figures/pca_slerp.png} % Specify width and maintain aspect ratio
   \caption{PCA -- Local-to-Parent Space}
    \label{fig:pca-local}
  \end{subfigure}
  \begin{subfigure}{0.23\textwidth}
    \centering
    \includegraphics[width=\textwidth, height=\textwidth, keepaspectratio]{figures/tsne_root.png} % Specify width and maintain aspect ratio
    \caption{t-SNE -- Root Space}
    \label{fig:tsne-root}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.23\textwidth}
    \centering
    \includegraphics[width=\textwidth, height=\textwidth, keepaspectratio]{figures/tsne_local_new.png} % Specify width and maintain aspect ratio
    \caption{t-SNE -- Local-to-Parent Space}
    \label{fig:tsne-local}
  \end{subfigure}
  \caption{Comparing root space (left) vs. local-to-parent space (right) features using 3D PCA (top) and 3D t-SNE (bottom). The colors indicate different actions in the test set. The legend can be found in the Appendix.}
  \label{fig:feature_rep}
\end{figure}

